How often should I access my online social networks?

Users of online social networks are faced with a conundrum of trying to be always informed without having enough time or attention budget to do so. The retention of users on online social networks has important implications, encompassing economic, psychological and infrastructure aspects. In this paper, we pose the following question: what is the optimal rate at which users should access a social network? To answer this question, we propose an analytical model to determine the value of an access (VoA) to the social network. In the simple setting considered in this paper, VoA is defined as the chance of a user accessing the network and obtaining new content. Clearly, VoA depends on the rate at which sources generate content and on the filtering imposed by the social network. Then, we pose an optimization problem wherein the utility of users grows with respect to VoA but is penalized by costs incurred to access the network. Using the proposed framework, we provide insights on the optimal access rate. Our results are parameterized using Facebook data, indicating the predictive power of the approach.

==> IEEECS_confs_LaTeX/README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> facebook.tex <==
\section{Facebook Experiments}

\subsection{Experimental setup}

explain Brazilian ellections and bots

\subsection{Post overlap}

intersection between posts

\subsection{Model parametrization with real data}



\begin{figure*}
    \centering
\begin{tabular}{cc}
     \includegraphics[width=0.5\textwidth]{VoA_FB_X_K.eps} &      \includegraphics[width=0.5\textwidth]{VoA_FB_X_mu.eps}  \\
     (a) & (b) 
     
\end{tabular}
%\vspace{-0.2in}
    \caption{VoA estimated using the fixed K model, the average K model, the Poisson K model and the measurements, (a) in function of $K$ and (b) in function of $\mu$   }
    \label{fig:totalpubs}
\end{figure*}


illustrate results





==> timeseries.tex <==
\section{Análise de séries temporais}
\label{sec:timeseries}

\section{Forecasting}
\label{sec:forecast}

\begin{figure*}
  \includegraphics[width=1.0\textwidth]{series_ocupacao.eps} 
\caption{Time series of occupation of the political orientations in the 6 users}
\label{fig:serietemporal_fontes}
\end{figure*}



Next, we study temporal aspects associated with timelines. Until that point, our focus was on the analysis of stationary metrics. In this section, we focused on the transient aspects of the publications featured in the top 10 News Feed positions of the 6 users participating in the experiment.

The figure \ref{fig:temporaltemporal_fontes} shows the evolution of the occupation of the sources over time in each of the six users. In this figure, the sources were grouped according to their respective political orientation to facilitate the visualization. The occupation values were smoothed by the \textit{geom\_smooth} function through the gam( Generalized Additive Models With Integrated Smoothness Estimation) \cite{GarrettGrolemund2016} function. This figure, in addition to confirming the observations made in Section~\ref{sec:italia}, shows that the center-left sources had an increase in occupation in all users from the beginning of March, and the left sources presented a peak occupancy in the left user in early February.

\begin{figure*}
  \includegraphics[width=1.0\textwidth]{series_ocupacao_M5S.eps} 
\caption{Série temporal da ocupação do movimento 5 estrelas (M5S) no usuário indeciso}
\label{fig:serietemporal_M5s}
\end{figure*}

To illustrate a time series of occupation of a source in a given News Feed, Figure ~\ref{fig:serietemporal_M5s} presents the occupation of the 5-Star Movement (M5S), the party that received the most votes in the 2018 Italian election in the user undecided Starting in early March, some snapshots even had $50\%$ of their positions occupied with 5-Star Movement publications. However, in general, there was little oscillation in the value of the average occupation.



Figure ~\ref{fig:seriepublicacoes} shows the ratio of the number of publications of the published policy guidelines over a period of time to the total number of publications made over the same period. The values of these fractions were also smoothed by the \textit{geom\_smooth} function through the gam method. The center-left and right-hand fonts were the ones that published the most content during the analyzed period, reinforcing the one indicated in Figure~\ref{fig:pubfontes}. It is important to note that the relative number of publications created by center-left sources decreases at the end of the analyzed period, while occupancy shows a sudden increase in all users in this period, as shown in Figure ~\ref{fig:temporaltemporal_fontes}.

\begin{figure*}
  \includegraphics[width=1.0\textwidth]{series_fontes.eps} 
\caption{Occupations time series of the selected publishers}
\label{fig:seriepublicacoes}
\end{figure*}

In particular, the analysis in this section is useful for both users and sources. From the users' point of view, it is useful to be able to predict, for example, the distribution of content in your timeline within a given future time window. Such a prediction serves, for example, to plan access to Facebook. Such planning, in turn, is useful for avoiding access to the system too often (which is costly in terms of attention) or very infrequently (possibly missing out on valuable information that is no longer at the top of the timeline  ).

From the point of view of sources, the possibility of predicting the distribution of content is useful for strategic purposes. Consider, for example, a source that chooses to strategically choose when to post content in such a way that your publications admit the least competition with publications from a source that produces a particular content type.

Figure ~\ref{fig previsoes} shows the prediction of occupation of the source \textit{La Repubblica} in the center-left user. The forecast is done in snapshot $ t + 1 $ using all occupancy values ​​from the first snapshot to snapshot $ t $. Using this forecast, a user may, for example, give up viewing their News Feed because the forecast indicates they will have few publications from a particular source in their next view. The predictions were made using the ARIMA model whose optimum parameters were calculated with the function \textit{auto\_arima ()} of the forecast package Forecast ~\cite{Hyndman2008} of R. The first forecast was made after collecting the first 60 snapshots. In Figure ~\ref{fig:previsoes}, the red dots represent the measurements, the blue predictions and the green ones, the errors. The solid lines represent smoothing of these points by the gam method of \textit {geom\_smooth}. Let $ \ hat {N} {ij} (t + 1) $ be the occupancy in the same snapshot $ t + 1 $ and $ N_ {ij}$ snapshot. The $ \epsilon (t + 1) $ error in the snapshot $ t + 1 $ is calculated by the absolute value of the difference between the measurement $ N_{ij} (t + 1) $ and the prediction $ \hat{N}_{ij}(t+1) $ according to the equation ~\eqref{eq:error}.

\begin{equation}
    \epsilon(t+1)=|\hat{N}_{ij}(t+1)-N_{ij}(t+1)|.
    \label{eq:erro}
\end{equation}

Figure ~\ref{fig:predictions} shows that the predictions followed the increase in the occupation of the center-left source at the end of the experiment period. Consequently, the error is approximately constant throughout the period and regardless of the size of the training set.








It should also be remembered that our model was parameterized using information about impressions. However, collecting impressions is costly. Web scrapping tools need to be developed and maintained in addition to the effort to manage the users involved in the experiments. In this way, ideally it is interesting to have a mechanism for predicting impressions from the source publication standard. In this section we present first steps in this direction. From the time series of publications of the sources we look for correlations between them and the series of impressions. Thus, in future work we envisage that it is possible to characterize (partially) the behavior of the timeline directly from publicly available information about sources (eg, publication creation standard) and users (eg, likes).


\begin{figure}
  \includegraphics[width=1.0\textwidth]{previsoes.eps} 
\caption{Prediction of occupancy in snapshot $t + 1$. The purple dots represent the predictions, the red dots the measured values and the green dots represent the errors
.}
\label{fig:previsoes}
\end{figure}
